Computational Approaches to Arabic-English Code-Switching

Natural Language Processing (NLP) is a vital computational method for addressing language processing, analysis, and generation. NLP tasks form the core of many daily applications, from automatic text correction to speech recognition. While significant research has focused on NLP tasks for the English language, less attention has been given to Modern Standard Arabic and Dialectal Arabic. Globalization has also contributed to the rise of Code-Switching (CS), where speakers mix languages within conversations and even within individual words (intra-word CS). This is especially common in Arab countries, where people often switch between dialects or between dialects and a foreign language they master. CS between Arabic and English is frequent in Egypt, especially on social media. Consequently, a significant amount of code-switched content can be found online. Such code-switched data needs to be investigated and analyzed for several NLP tasks to tackle the challenges of this multilingual phenomenon and Arabic language challenges. No work has been done before for several integral NLP tasks on Arabic-English CS data. In this work, we focus on the Named Entity Recognition (NER) task and other tasks that help propose a solution for the NER task on CS data, e.g., Language Identification. This work addresses this gap by proposing and applying state-of-the-art techniques for Modern Standard Arabic and Arabic-English NER. We have created the first annotated CS Arabic-English corpus for the NER task. Also, we apply two enhancement techniques to improve the NER tagger on CS data using CS contextual embeddings and data augmentation techniques. All methods showed improvements in the performance of the NER taggers on CS data. Finally, we propose several intra-word language identification approaches to determine the language type of a mixed text and identify whether it is a named entity or not.

==> Data_Collection_annotation.tex <==
\chapter{Corpora Generation}\label{chap:cscorpus}
\section{Code-Mixed Named Entity Corpus}
We present our code-switched corpus which is an extension to our work in \cite{sabty2019named}. The corpus is composed of 6,525 sentences that contains 136,574 tokens. It has 22,705 (16.6\%) English words and 113,869 (83.4\%) Arabic words. The data was gathered through three different sources. The first one is collecting 2,303 Egyptian-English CM sentences from Twitter. The second one is taking 1,150 sentences from the transcribed speech corpus for conversational Egyptian Arabic \cite{hamed2018collection}. The last one is translating 3,072 sentences from the Arabic ANERCorp and AQMAR data-sets for Named Entity Recognition.

After collecting the data, the annotation of the entities started by identifying the boundaries of the named entity and then assigning the correct NE type. Our annotations followed the Named Entity Annotation guidelines for the shared task of CoNLL-2003 \cite{tjong2003introduction}. It is concerned with four types of entities: persons (PER), locations (LOC), organizations (ORG) and names of miscellaneous (MISC), that do not belong to any of the three types. Words that are not named entities are tagged with O. 
\begin{table}[!ht]
\centering
\begin{tabular}{||l | r||} 
\hline
\textbf{Data-set} & \textbf{No. of Sentences }\\ [0.5ex] 
\hline\hline
Twitter & 1,477 (64.1\%) \\
Translated & 3,059 (99.6\%) \\ 
Transcribed Speech  & 412 (35.8\%) \\ 
\textbf{Total} & 4,948 (75.8\%) \\ \hline
\end{tabular}
\caption{ Number of sentences containing entities in each data-set}
\label{table:total}
\end{table}


Table \ref{table:total} shows the number of sentences containing entities in each data-set and their percentages. The total number of sentences in the corpus containing entities is 4,948 sentences, which is 75.8\% from the total number of sentences. 

The total number of NEs in the corpus is 17,577 tokens. Table \ref{table:totalInClass} shows the total number of words under each NE class. The person class contains the highest number of entities which is  6,534 entities and the organization class contains the minimum number of entities which is 3,100 entities.

\begin{table}[!ht]
\centering
\begin{tabular}{||l | r| r||} 
\hline
\textbf{Entity Type} & \textbf{Words} & \textbf{\% of Total Words }\\ [0.5ex] 
\hline\hline
Person & 6,534 & 4.8  \\ 
Location & 4,219 & 3.1 \\ 
Organization & 3,100 & 2.3\\ 
Miscellaneous & 3,724 & 2.7 \\ 
\textbf{Total entities}  & 17,577 & 12.9\\\hline \end{tabular}
\caption{ Number of entities in each entity type in the final data-set}
\label{table:totalInClass}
\end{table}



\subsection{Twitter Data-set}
The first part of the corpus is composed of data harvested from Twitter by querying the Twitter API\footnote{https://developer.twitter.com/en/docs/api-reference-index}. We implemented different approaches to collect tweets containing CM data. In the first phase of collection, one of the approaches was randomly selecting some tweets by gathering them using a query requiring the tweets to have a hash tag. A big percentage of the hash tags are written in the English language. The tokenization of the hash tags is automatically done while collecting the tweets. Moreover, the query required that the tweets should contain Arabic language. Another filtering criteria was done by checking that the tweets contain at least two English words to guarantee that the sentence contains CM text. However, words such as http or via were not counted.

In the second phase of collection, other techniques were used to search for tweets that contain named entities. We used some of the named entities found in ANERCorp data set as keywords in the search queries to collect more tweets containing NEs. Moreover, in order to guarantee having sentences containing entities, we created a list of names of famous persons and used them as seeds to collect tweets. 

The total number of collected sentences using Twitter is 2,303 sentences which contains 38,281 tokens. As shown in Table \ref{table:twitter}, this part of the corpus has 5,810 entities which is 15.2\% from the total number of words. It consists of 7,405 (19.3\%) English words and 30,876 (80.7\%) Arabic words. We can observe that the miscellaneous class contains the highest number of entities and the location class contains the lowest number of entities.
\begin{table}[!ht]
\centering
\begin{tabular}{||l | r| r||} 
\hline
\textbf{Entity Type} & \textbf{Words} & \textbf{\% of Total Words} \\ [0.5ex] 
\hline\hline
Person& 1,907 & 5.0 \\
Location & 550 & 1.4 \\
Organization & 1,098 & 2.9\\
Miscellaneous & 2,255 & 5.9 \\
\textbf{Total entities}  & 5,810 & 15.2 \\\hline \end{tabular}
\caption{Number of entities in each entity type in the Twitter data-set}
\label{table:twitter}
\end{table}



\subsection{Translated Data-Set}
The second part is gathered by translating some of the existing annotated Arabic NER data. In the first collection phase, the selected sentences were randomly chosen from the Arabic ANERCorp data-set. In some sentences, we translated all the entities they contained. Other sentences we translated one or two entities only, in order to have Arabic entities in addition to the English entities in this part of the corpus. During the second phase of collection more sentences were chosen from the same data-set in addition, to sentences selected from AQmar data-set. 

This technique was time efficient as there was no need to annotate the data. However, sometimes it did not generate correct translations for miscellaneous or organization entities as they might have several meanings. Thus, a manual check was done on data to ensure that the words were translated correctly.

The number of translated sentences is 3,072 sentences which contains 78,215 tokens. They are composed of 8,549 (10.9\%) English words and 69,666 (89.1\%) Arabic words. As shown in Table \ref{table:translated}, the total number of named entities it has is 11,391 which is 14.6\% of the total number of words. The person class contains the highest number of words which is equal to 4,516 words, and the miscellaneous class contains the minimum number of words which is equal to 1,348 words.

\begin{table}[!ht]
\centering
\begin{tabular}{||l | r| r||} 
\hline
\textbf{Entity Type} & \textbf{Words} & \textbf{\% of Total Words}  \\ [0.5ex] 
\hline\hline
Person& 4,516 & 5.8\\
Location & 3,601 & 4.6 \\
Organization & 1,926 & 2.5 \\
Miscellaneous & 1,348 & 1.7  \\
\textbf{Total entities}  & 11,391 & 14.6 \\\hline \end{tabular}
\caption{Number of entities in each entity type in the translated data-set}
\label{table:translated}
\end{table}




\subsection{Transcribed Speech Data-set}
The third part of our corpus is composed of data from the transcribed speech data-set \cite{hamed2018collection}. They gathered spontaneous speech through informal interviews. The interviews topics were technical ones to have a higher probability to contain CM. They manually transcribed the corpus and they formed
a total of 1,234 sentences and 17,769 tokens. In the original speech corpus the sentences were divided into 124 monolingual Arabic,
125 monolingual English and 985 mixed. Overall, the data-set contains 79.8\% of code-mixing, 10.1\% of code-switching and 10\% of purely Arabic.

\begin{table}[!ht]
\centering
\begin{tabular}{||l | r| r||} 
\hline
\textbf{Entity Type} & \textbf{Tokens} & \textbf{\% of Total Words}  \\ [0.5ex] 
\hline\hline
Person & 111 & 0.6 \\
Location & 68 & 0.3 \\
Organization & 76 & 0.4 \\
Miscellaneous & 121 & 0.6 \\
\textbf{Total entities}   & 376 & 1.9 \\\hline \end{tabular}
\caption{Number of entities in each entity type in the transcribed speech data-set}
\label{table:speech}
\end{table}

As shown in Table \ref{table:speech}, this part of the corpus contains 1,150 sentences containing 20,078 tokens. As some pre-processings were performed on the data and added more tokens/sentences. It has 13,327 (66.4\%) Arabic and 6,751 (33.6\%) English words. The miscellaneous class contains the maximum number of entities which is equal to 121 words and the location is the lowest which is equal to 68 words only.
\subsection{Data Annotation}

The annotation of the entities started by identifying the boundaries of the named entity and then assigning the correct NE type. 
Our annotations followed the Named Entity Annotation guidelines for the shared task of CoNLL-2003 \cite{tjong2003introduction}. It is concerned with four types of entities: persons (PER), locations (LOC), organizations (ORG) and names of miscellaneous (MISC), that do not belong to any of the three types. Words that are not named entities are tagged with O. It also follows the IOB scheme  \cite{sang1999representing}. 
%Words tagged with O are outside of named entities
%and the I-XXX tag is used for words inside a
%named entity of type XXX. Whenever two entities of
%type XXX are immediately next to each other, the
%first word of the second entity will be tagged B-XXX
%in order to show that it starts another entity. The
%data contains entities of four types: persons (PER),
%organizations (ORG), locations (LOC) and miscellaneous
%names (MISC). This tagging scheme is the
%IOB scheme originally put forward by Ramshaw and
%Marcus (1995).
\section{Language Identification Corpus}

\section{Games With a Purpose for Data Collection}


==> Discussion.tex <==
\chapter{Results \& Discussion}\label{chap:results}
